HDR-Polar1K: An HDR Stokes Image Dataset for Learning Color-Polarization Reconstruction

Color-polarization filter array (CPFA) cameras require joint demosaicing and denoising to recover dense color Stokes images from RAW measurements. Existing training datasets are limited by acquisition artifacts and insufficient coverage of controlled optical scenes. We introduce HDR-Polar1K, a dataset of 1,008 HDR color Stokes images spanning everyday and controlled scenes. Repeated, exposure-bracketed CPFA capture and CPFA-aware downsampling produce images free of saturation and nonphysical Stokes vectors. These HDR images enable brightness variation and calibrated sensor simulation for training under diverse sensor conditions. Training on HDR-Polar1K improves reconstruction across multiple networks. We also introduce Raw2Stokes, which produces physically valid Stokes images with optional sensor conditioning. Trained on HDR-Polar1K using our calibrated sensor simulation, Raw2Stokes enables practical color-polarization reconstruction from full-resolution real RAW captures.

==> preamble.tex <==
\usepackage{iftex}
\ifPDFTeX
\usepackage[accsupp]{axessibility}
\fi
\usepackage{graphicx}
\makeatletter
\newcommand{\PaperSRGBRasters}{%
  \@ifundefined{PaperSRGBSpace}{%
    \immediate\pdfobj stream attr{/N 3 /Alternate /DeviceRGB} file{figures/paper-srgb.icc}%
    \immediate\pdfobj{[/ICCBased \the\pdflastobj\space 0 R]}%
    \xdef\PaperSRGBSpace{\the\pdflastobj}%
  }{}%
  \def\Gread@png##1{%
    \let\Gin@page\@empty
    \def\Gin@pagebox{\space}%
    \let\PaperOriginalXImage\pdfximage
    \def\pdfximage{\PaperOriginalXImage colorspace \PaperSRGBSpace\space}%
    \Gread@pdftex{##1}}%
  \let\Gread@jpg\Gread@png}
\makeatother
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{CJKutf8}
\usepackage{array}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage[dvipsnames]{xcolor}
\usepackage{breakcites}
\usepackage{url}
\usepackage{colortbl}
\usepackage{nccmath}
\usepackage{makecell}
\usepackage{times}
\usepackage{epsfig}
\usepackage{relsize}
\usepackage{algpseudocode}
\usepackage[ruled]{algorithm2e}
\usepackage{wrapfig}
\usepackage{soul}
\usepackage{calc}

\renewcommand{\algorithmcfname}{ALGORITHM}
\SetKwComment{Comment}{/* }{ */}
\captionsetup[subfigure]{format=hang}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}



\newcolumntype{Y}{>{\centering\arraybackslash}X}

\expandafter\def\csname ArxivImage:figures/controlled-scene-setups/color-filters.jpg\endcsname#1{\includegraphics[#1]{figures/controlled-scene-setups/color-filters.jpg}}
\expandafter\def\csname ArxivImage:figures/controlled-scene-setups/display-illumination.jpg\endcsname#1{\includegraphics[#1]{figures/controlled-scene-setups/display-illumination.jpg}}
\expandafter\def\csname ArxivImage:figures/controlled-scene-setups/display.jpg\endcsname#1{\includegraphics[#1]{figures/controlled-scene-setups/display.jpg}}
\expandafter\def\csname ArxivImage:figures/controlled-scene-setups/photoelastic-setup-zoom.jpg\endcsname#1{\includegraphics[#1]{figures/controlled-scene-setups/photoelastic-setup-zoom.jpg}}
\expandafter\def\csname ArxivImage:figures/controlled-scene-setups/photoelastic-setup.jpg\endcsname#1{\includegraphics[#1]{figures/controlled-scene-setups/photoelastic-setup.jpg}}
\expandafter\def\csname ArxivImage:figures/controlled-scene-setups/pink-filtered-light.jpg\endcsname#1{\includegraphics[#1]{figures/controlled-scene-setups/pink-filtered-light.jpg}}
\expandafter\def\csname ArxivImage:figures/controlled-scene-setups/polarizer.jpg\endcsname#1{\includegraphics[#1]{figures/controlled-scene-setups/polarizer.jpg}}
\expandafter\def\csname ArxivImage:figures/controlled-scene-setups/polarizing-sheet.jpg\endcsname#1{\includegraphics[#1]{figures/controlled-scene-setups/polarizing-sheet.jpg}}
\expandafter\def\csname ArxivImage:figures/controlled-scene-setups/projector.jpg\endcsname#1{\includegraphics[#1]{figures/controlled-scene-setups/projector.jpg}}
\expandafter\def\csname ArxivImage:figures/cpfa-intro-panels/s0.png\endcsname#1{\includegraphics[#1]{figures/cpfa-intro-panels/s0.png}}
\expandafter\def\csname ArxivImage:figures/cpfa-intro-panels/s1.png\endcsname#1{\includegraphics[#1]{figures/cpfa-intro-panels/s1.png}}
\expandafter\def\csname ArxivImage:figures/cpfa-intro-panels/s2.png\endcsname#1{\includegraphics[#1]{figures/cpfa-intro-panels/s2.png}}
\expandafter\def\csname ArxivImage:figures/hdr-reference-correction-panels/legend-aolp.png\endcsname#1{\includegraphics[#1]{figures/hdr-reference-correction-panels/legend-aolp.png}}
\expandafter\def\csname ArxivImage:figures/hdr-reference-correction-panels/legend-dolp.png\endcsname#1{\includegraphics[#1]{figures/hdr-reference-correction-panels/legend-dolp.png}}
\expandafter\def\csname ArxivImage:figures/hdr-reference-correction-panels/roi2-baseline-aolp.png\endcsname#1{\includegraphics[#1]{figures/hdr-reference-correction-panels/roi2-baseline-aolp.png}}
\expandafter\def\csname ArxivImage:figures/hdr-reference-correction-panels/roi2-baseline-dolp.png\endcsname#1{\includegraphics[#1]{figures/hdr-reference-correction-panels/roi2-baseline-dolp.png}}
\expandafter\def\csname ArxivImage:figures/hdr-reference-correction-panels/roi2-baseline-s0.png\endcsname#1{\includegraphics[#1]{figures/hdr-reference-correction-panels/roi2-baseline-s0.png}}
\expandafter\def\csname ArxivImage:figures/hdr-reference-correction-panels/roi2-dark_masked-aolp.png\endcsname#1{\includegraphics[#1]{figures/hdr-reference-correction-panels/roi2-dark_masked-aolp.png}}
\expandafter\def\csname ArxivImage:figures/hdr-reference-correction-panels/roi2-dark_masked-dolp.png\endcsname#1{\includegraphics[#1]{figures/hdr-reference-correction-panels/roi2-dark_masked-dolp.png}}
\expandafter\def\csname ArxivImage:figures/hdr-reference-correction-panels/roi2-dark_masked-s0.png\endcsname#1{\includegraphics[#1]{figures/hdr-reference-correction-panels/roi2-dark_masked-s0.png}}
\expandafter\def\csname ArxivImage:figures/hdr-reference-correction-panels/roi2-detail-raw.png\endcsname#1{\includegraphics[#1]{figures/hdr-reference-correction-panels/roi2-detail-raw.png}}
\expandafter\def\csname ArxivImage:figures/hdr-reference-correction-panels/roi2-hdr-raw.png\endcsname#1{\includegraphics[#1]{figures/hdr-reference-correction-panels/roi2-hdr-raw.png}}
\expandafter\def\csname ArxivImage:figures/main-real-jdd-panels/legend-aolp.png\endcsname#1{\includegraphics[#1]{figures/main-real-jdd-panels/legend-aolp.png}}
\expandafter\def\csname ArxivImage:figures/main-real-jdd-panels/legend-dolp.png\endcsname#1{\includegraphics[page=14,#1]{figures/supp-real-172815-panels.pdf}}
\expandafter\def\csname ArxivImage:figures/main-reference-construction-ball-panels/hdr.png\endcsname#1{\includegraphics[#1]{figures/main-reference-construction-ball-panels/hdr.png}}
\expandafter\def\csname ArxivImage:figures/main-reference-construction-ball-panels/raw-0.png\endcsname#1{\includegraphics[#1]{figures/main-reference-construction-ball-panels/raw-0.png}}
\expandafter\def\csname ArxivImage:figures/main-reference-construction-ball-panels/raw-2.png\endcsname#1{\includegraphics[#1]{figures/main-reference-construction-ball-panels/raw-2.png}}
\expandafter\def\csname ArxivImage:figures/main-reference-construction-ball-panels/raw-5.png\endcsname#1{\includegraphics[#1]{figures/main-reference-construction-ball-panels/raw-5.png}}
\expandafter\def\csname ArxivImage:figures/main-reference-construction-ball-panels/s0.png\endcsname#1{\includegraphics[#1]{figures/main-reference-construction-ball-panels/s0.png}}
\expandafter\def\csname ArxivImage:figures/main-reference-construction-ball-panels/s1.png\endcsname#1{\includegraphics[#1]{figures/main-reference-construction-ball-panels/s1.png}}
\expandafter\def\csname ArxivImage:figures/main-reference-construction-ball-panels/s2.png\endcsname#1{\includegraphics[#1]{figures/main-reference-construction-ball-panels/s2.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/exposure_001.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/exposure_001.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/exposure_01.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/exposure_01.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/exposure_1.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/exposure_1.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/gain_0.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/gain_0.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/gain_24.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/gain_24.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/gain_48.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/gain_48.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/ideal_mosaic.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/ideal_mosaic.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/reference_s0.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/reference_s0.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/temperature_50.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/temperature_50.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/temperature_60.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/temperature_60.png}}
\expandafter\def\csname ArxivImage:figures/sensor-degradation-panels/temperature_70.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/temperature_70.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/bird-high-crop.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/bird-high-crop.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/bird-high.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/bird-high.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/bird-low-crop.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/bird-low-crop.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/bird-low.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/bird-low.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/bird-thermal-crop.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/bird-thermal-crop.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/bird-thermal.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/bird-thermal.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/dolls-high-crop.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/dolls-high-crop.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/dolls-high.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/dolls-high.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/dolls-low-crop.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/dolls-low-crop.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/dolls-low.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/dolls-low.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/dolls-thermal-crop.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/dolls-thermal-crop.png}}
\expandafter\def\csname ArxivImage:figures/sensor-test-conditions/dolls-thermal.png\endcsname#1{\includegraphics[#1]{figures/sensor-test-conditions/dolls-thermal.png}}
\expandafter\def\csname ArxivImage:figures/supp-construction-intensities/i0.png\endcsname#1{\includegraphics[#1]{figures/supp-construction-intensities/i0.png}}
\expandafter\def\csname ArxivImage:figures/supp-construction-intensities/i135.png\endcsname#1{\includegraphics[#1]{figures/supp-construction-intensities/i135.png}}
\expandafter\def\csname ArxivImage:figures/supp-construction-intensities/i45.png\endcsname#1{\includegraphics[#1]{figures/supp-construction-intensities/i45.png}}
\expandafter\def\csname ArxivImage:figures/supp-construction-intensities/i90.png\endcsname#1{\includegraphics[#1]{figures/supp-construction-intensities/i90.png}}
\expandafter\def\csname ArxivImage:figures/supp-print-overviews/raw-0.png\endcsname#1{\includegraphics[#1]{figures/supp-print-overviews/raw-0.png}}
\expandafter\def\csname ArxivImage:figures/supp-print-overviews/raw-2.png\endcsname#1{\includegraphics[#1]{figures/supp-print-overviews/raw-2.png}}
\expandafter\def\csname ArxivImage:figures/supp-print-overviews/raw-5.png\endcsname#1{\includegraphics[#1]{figures/supp-print-overviews/raw-5.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-with-A-AoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-with-A-AoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-with-A-DoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-with-A-DoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-with-A-S0.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-with-A-S0.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-with-C-AoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-with-C-AoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-with-C-DoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-with-C-DoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-with-C-S0.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-with-C-S0.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-without-A-AoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-without-A-AoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-without-A-DoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-without-A-DoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-without-A-S0.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-without-A-S0.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-without-C-AoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-without-C-AoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-without-C-DoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-without-C-DoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/bird-without-C-S0.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/bird-without-C-S0.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-with-A-AoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-with-A-AoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-with-A-DoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-with-A-DoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-with-A-S0.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-with-A-S0.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-with-C-AoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-with-C-AoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-with-C-DoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-with-C-DoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-with-C-S0.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-with-C-S0.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-without-A-AoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-without-A-AoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-without-A-DoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-without-A-DoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-without-A-S0.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-without-A-S0.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-without-C-AoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-without-C-AoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-without-C-DoLP.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-without-C-DoLP.png}}
\expandafter\def\csname ArxivImage:figures/supp-real-training-noise/day-without-C-S0.png\endcsname#1{\includegraphics[#1]{figures/supp-real-training-noise/day-without-C-S0.png}}
\expandafter\def\csname ArxivImage:figures/supp-sensor-flow-panels/s0.png\endcsname#1{\includegraphics[#1]{figures/sensor-degradation-panels/reference_s0.png}}
\expandafter\def\csname ArxivImage:figures/supp-sensor-flow-panels/s1.png\endcsname#1{\includegraphics[#1]{figures/supp-sensor-flow-panels/s1.png}}
\expandafter\def\csname ArxivImage:figures/supp-sensor-flow-panels/s2.png\endcsname#1{\includegraphics[#1]{figures/supp-sensor-flow-panels/s2.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/gt-aolp.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/gt-aolp.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/gt-dolp.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/gt-dolp.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/gt-s0.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/gt-s0.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/high-clean-aolp.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/high-clean-aolp.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/high-clean-dolp.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/high-clean-dolp.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/high-clean-s0.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/high-clean-s0.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/high-simulated-aolp.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/high-simulated-aolp.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/high-simulated-dolp.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/high-simulated-dolp.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/high-simulated-s0.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/high-simulated-s0.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/low-clean-aolp.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/low-clean-aolp.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/low-clean-dolp.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/low-clean-dolp.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/low-clean-s0.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/low-clean-s0.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/low-simulated-aolp.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/low-simulated-aolp.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/low-simulated-dolp.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/low-simulated-dolp.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-sensor-noise/low-simulated-s0.png\endcsname#1{\includegraphics[#1]{figures/supp-training-sensor-noise/low-simulated-s0.png}}
\expandafter\def\csname ArxivImage:figures/supp-training-set-size/mae_aolp_degrees.pdf\endcsname#1{\includegraphics[#1]{figures/supp-training-set-size/mae_aolp_degrees.pdf}}
\expandafter\def\csname ArxivImage:figures/supp-training-set-size/mae_dolp_clipped.pdf\endcsname#1{\includegraphics[#1]{figures/supp-training-set-size/mae_dolp_clipped.pdf}}
\expandafter\def\csname ArxivImage:figures/supp-training-set-size/mse.pdf\endcsname#1{\includegraphics[#1]{figures/supp-training-set-size/mse.pdf}}
\expandafter\def\csname ArxivImage:figures/training-data-barplots/low-noise-trim5-mae_aolp_degrees.pdf\endcsname#1{\includegraphics[#1]{figures/training-data-barplots/low-noise-trim5-mae_aolp_degrees.pdf}}
\expandafter\def\csname ArxivImage:figures/training-data-barplots/low-noise-trim5-mae_dolp_clipped.pdf\endcsname#1{\includegraphics[#1]{figures/training-data-barplots/low-noise-trim5-mae_dolp_clipped.pdf}}
\expandafter\def\csname ArxivImage:figures/training-data-barplots/low-noise-trim5-mse.pdf\endcsname#1{\includegraphics[#1]{figures/training-data-barplots/low-noise-trim5-mse.pdf}}
\expandafter\def\csname ArxivImage:figures/training-data-barplots/low-noise-trim5-nonphysical_percent.pdf\endcsname#1{\includegraphics[#1]{figures/training-data-barplots/low-noise-trim5-nonphysical_percent.pdf}}

